A survey of Community Question Answering

With the advent of numerous community forums, tasks associated with the same have gained importance in the recent past. With the influx of new questions every day on these forums, the issues of identifying methods to find answers to said questions, or even trying to detect duplicate questions, are of practical importance and are challenging in their own right. This paper aims at surveying some of the aforementioned issues, and methods proposed for tackling the same.

==> DiffFromQA.tex <==
\section{Community QA vs QA} \label{sec:DiffFromQA}
\begin{figure*}[ht]
{\footnotesize
%\begin{adjustwidth}{-2.2cm}{}
%  Requires \usepackage{graphicx}
\center
  \includegraphics[scale=0.35]{figs/queryExample3.jpg}
  \caption{Question from an online tourism forum and its corresponding semantic representation.}\label{fig:queryExample}
%\end{adjustwidth}
}
\vspace*{-3ex}
\end{figure*}

==> Introduction.tex <==
\section{Introduction} \label{sec:Introduction}
Community Question Answering has seen a spectacular increase in popularity in the recent past. With the advent and popularity of sites like Yahoo! Answers\footnote{https://answers.yahoo.com}, Cross Validated\footnote{http://stats.stackexchange.com/}, Stack Overflow\footnote{https://www.stackoverflow.com}, Quora\footnote{https://www.quora.com/}, more and more people now use these web forums to get answers to their questions. These forums give people the ability to post their queries online, and have multiple experts across the world answer them, while being able to provide their opinions or expertise to help other users, a quality that encourages more participation and consequently has lead to their popularity.     \\
This survey aims at discussing some of the challenges that accompany such community forums, and the way they have been approached. Section 2 defines the attributes of community question answering and contrasts it with the traditional question answering task. Section 3 defines some of the tasks seen in this domain and also investigates the methods used to solve them and the results obtained. Section 4 then speaks about some of the datasets available for the aforementioned tasks as well as a note on the quality of questions in such forums. Finally, section 5 concludes this survey.

